BIMBA: Selective-Scan Compression for Long-Range Video Question Answering

Video Question Answering (VQA) in long videos poses the key challenge of extracting relevant information and modeling long-range dependencies from many redundant frames. The self-attention mechanism provides a general solution for sequence modeling, but it has a prohibitive cost when applied to a massive number of spatiotemporal tokens in long videos. Most prior methods rely on compression strategies to lower the computational cost, such as reducing the input length via sparse frame sampling or compressing the output sequence passed to the large language model (LLM) via space-time pooling. However, these naive approaches over-represent redundant information and often miss salient events or fast-occurring space-time patterns. In this work, we introduce BIMBA, an efficient state-space model to handle long-form videos. Our model leverages the selective scan algorithm to learn to effectively select critical information from high-dimensional video and transform it into a reduced token sequence for efficient LLM processing. Extensive experiments demonstrate that BIMBA achieves state-of-the-art accuracy on multiple long-form VQA benchmarks, including PerceptionTest, NExT-QA, EgoSchema, VNBench, LongVideoBench, and Video-MME. Code, and models are publicly available at https://sites.google.com/view/bimba-mllm.

==> tables/compression_methods.tex <==
\begin{table}[]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Compression\\ Method\end{tabular}}} & \multicolumn{2}{c}{\modelLlava} & \multicolumn{2}{c}{\modelLlama} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multicolumn{1}{c}{}  & NextQA & EgoSchema & NextQA & EgoSchema \\ 
\toprule
Vanilla  & 67.16       & 50.13          & 72.77        & 58.23      \\
Pooling   & 68.85       & 52.78          & 71.27        & 57.16     \\
Self-Attention  & 69.61       & 53.61          & 72.16    & 54.19  \\
Perceiver  & 70.23       & 54.21          & 73.41        & 56.13  \\
BIMBA  & \textbf{73.57}       & \textbf{58.40}          & \textbf{75.57}        & \textbf{62.20}          \\ 
\bottomrule
\end{tabular}
}
\caption{Comparison Between Different Compression Methods.}
\label{tab:compression}
\end{table}

==> tables/main_results1.tex <==
\begin{table*}[t]
\vspace{-5mm}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
Model & LLM & Frames & PerceptionTest & NExT-QA & EgoSchema & VNBench & LongVideoBench & Video-MME & MLVU \\
Duration & & & 23 sec & 44 sec & 180 sec & 180 sec & 8 sec - 60 min & 1 - 60 min & 3 - 120 min \\
\toprule
\rowcolor{lightgray}\multicolumn{10}{c}{(Based on Proprietary LLMs)} \\
LLoVi~\cite{zhang2023simple} & GPT3.5 & - & - & 66.30 & 52.00 & - & - & - & - \\
VideoAgent~\cite{wang2024videoagent} & GPT4 & - & - & 71.30 & 54.10 & - & - & - & - \\
VideoTree~\cite{wang2024videotree} & GPT4 & - & - & 75.60 & 61.10 & - & - & - & - \\
\rowcolor{lightgray}\multicolumn{10}{c}{(Open-source MLLMs Trained on Our 370K Video Instruction Data)} \\
LLaVA-NeXT (Video)~\cite{liu2024llavanext} & Vicuna-7B & 64 & 46.13 & 67.66 & 41.66 & - & - & 42.21 & 42.33 \\
PLLaVA~\cite{xu2024pllavaparameterfreellava} & Vicuna-7B & 64 & 48.55 & 67.56 & 43.36 & - & - & 42.13 & 44.61 \\
\textbf{\modelLlava} & Vicuna-7B & 64 & 52.61 & 72.35 & 52.31 & - & - & 45.66 & 47.16 \\
\hline
LLaMA-3.2 (Video)~\cite{llama3.2} & LLaMA3.2-8B & 64 & 53.16 & 73.72 & 55.21 & - & - & 47.31 & 47.61 \\
PLLaVA (LLaMA-3.2)~\cite{llama3.2} & LLaMA3.2-8B & 64 & 53.13 & 72.77 & 52.33 & - & - & 46.56 & 46.56 \\
\textbf{\modelLlama} & LLaMA3.2-8B & 64 & 56.50 & 76.88 & 60.25 & - & - & 50.11 & 50.60 \\
\rowcolor{lightgray}\multicolumn{10}{c}{(Open-source MLLMs Trained on Larger Scale Instruction Video Data)} \\
LLaMA-VID~\cite{Li2023LLaMAVIDAI} & Vicuna-7B & 1fps & 44.60 & - & 38.50 & 10.80 & - & - & 33.20 \\
Video-LLaVA~\cite{lin2023video} & Vicuna-7B & 8 & 44.30 & 62.60 & 38.40 & - & - & 40.40 & 47.30 \\
LLaVA-NeXT-Video~\cite{zhang2024llavanextvideo} & Vicuna-7B & 32 & 48.80 & - & 43.90 & 20.10 & 43.50 & 46.50 & - \\
PLLaVA~\cite{xu2024pllavaparameterfreellava} & Vicuna-7B & 16 & - & 68.17 & 45.16 & - & 40.20 & 44.25 & 47.31 \\
VideoChat2~\cite{li2023mvbench} & Vicuna-7B & 16 & 47.30 & - & 54.40 & 12.40 & 36.00 & 47.90 & 54.60 \\
LongVA~\cite{zhang2024long} & Qwen2-7B & 128 & - & 68.30 & - & 41.50 & - & 54.30 & 56.30 \\
Video-LLaMA2~\cite{cheng2024videollama} & Qwen2-7B & 32 & 51.40 & - & 51.70 & 24.90 & - & 47.90 & 48.50 \\
LLaVA-OneVision~\cite{li2024llava} & Qwen2-7B & 32 & 57.10 & 79.40 & 60.10 & 51.80 & 56.5 & 58.20 & 64.70 \\
Kangaroo~\cite{liu2024kangaroo} & LLaMA2-8B & 64 & - & - & 62.70 & - & - & 56.00 & 61.00 \\
Video-XL~\cite{shu2024video} & Qwen2-7B & 2048 & - & - & - & 61.60 & 49.50 & 55.50 & 64.90 \\
LongVU~\cite{shen2024longvu} & Qwen2-7B & 1fps & - & - & 67.60 & - & - & 60.60 & 65.40 \\
Qwen2-VL~\cite{wang2024qwen2} & Qwen2-7B & 2fps & - & - & - & - & 55.60 & 63.30 & - \\
LLaVA-Video~\cite{zhang2024video} & Qwen2-7B & 64 & 67.90 & 83.20 & 57.30 & 70.77 & 58.20 & 63.30 & 70.80 \\
\textbf{\modelLlava} & Qwen2-7B & 128 & \textbf{68.51} & \textbf{83.73} & \textbf{71.14} & \textbf{77.88} & \textbf{59.46} & \textbf{64.67} & \textbf{71.37} \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{We compare \model\ with state-of-the-art video MLLMs across seven diverse video question-answering benchmarks. \modelLlava\ achieves the highest performance on all datasets when using the Qwen2-7B LLM backbone (third section). Since different MLLMs leverage varying LLM backbones and training data, we also conduct a fair comparison by evaluating our model against four baselines trained using the same 370K instruction-tuning dataset and using Vicuna-7B and LLaMA3.2-8B LLM decoders (second section). In this evaluation setting, we observe that our model consistently outperforms all baselines across all benchmarks.}
\vspace{-5mm}
\label{tab:main result}
\end{table*}

==> tables/s6.tex <==
\begin{table}
  \caption{}
  \small
  \centering
  \resizebox{0.5\textwidth}{!}{%
  \begin{tabular}{@{}lllll@{}}
    \toprule & Convolution & Recurrence   & Self-Attention  & State-Space  \\
    \midrule
    Parameters & \( LH \)                                                                                                                                             & \( \bm{H^2} \) & \( \bm{H^2} \)       & \( \bm{H^2} \)                             \\
    Parallel   & \textbf{Yes}                                                                                                                                         & No             & \textbf{Yes}         & \textbf{Yes}                                     \\
    Memory      & \( \bm{BLH} \)                                                                                                                                       & \( \bm{BLH} \) & \( B(L^2 + HL) \)    & \( \bm{BLH} \)                                   \\
    Training Time  & \( \bm{\tilde{L}H(B + H)} \)                                                                                                                         & \( BLH^2 \)    & \( B(L^2H + LH^2) \) & \( \bm{BH(\tilde{H}+\tilde{L}) + B\tilde{L}H} \) \\
    Inference Time & \( LH^2 \)                                                                                                                                           & \( \bm{H^2} \) & \( L^2H + H^2L \)    & \( \bm{H^2} \)                                   \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:ssm}
\end{table}
